Empowerment-driven Exploration using Mutual Information Estimation

Exploration is a difficult challenge in reinforcement learning and is of prime importance in sparse reward environments. However, many of the state of the art deep reinforcement learning algorithms, that rely on epsilon-greedy, fail on these environments. In such cases, empowerment can serve as an intrinsic reward signal to enable the agent to maximize the influence it has over the near future. We formulate empowerment as the channel capacity between states and actions and is calculated by estimating the mutual information between the actions and the following states. The mutual information is estimated using Mutual Information Neural Estimator and a forward dynamics model. We demonstrate that an empowerment driven agent is able to improve significantly the score of a baseline DQN agent on the game of Montezuma's Revenge.

==> methods.tex <==
%!TEX root = ../effemp.tex
\section{Methods}
\label{sec:methods}
We consider a dynamical system over sequences $\bstateTs$ subject to control inputs $\bactionTs$.
The first state $\bstate_1$ is drawn from the \emph{initial state distribution} $\initial$; subsequently control inputs and successor states are drawn alternatingly from some \emph{policy} $\policy{\baction_t}{\bstate_t}$  and the \emph{transition distribution} $\p{\bstate_{t+1}}{\bstatet, \bactiont}$.
The complete likelihood is hence given as
\eq{
    \p{\bstateTs, \bactionTs} = \initial{\bstate_1} \prod_{t=1}^T\p{\bstate_{t+1}}{\bstate_t, \baction_t}\,\policy{\baction_t}{\bstate_t}. \numberthis \label{eq:joint_dynamics}
}
Note that we consider the state transition to be Markovian, \ie $\bstate_{t+1}$ is conditionally independent of $\bstate_{1:t-1}$ and $\baction_{1:t-1}$ given $\bstate_t$ and $\baction_t$. In the following we also use $\nowstate$ and $\succstate$ to denote $\bstate_t$ and its successor state $\bstate_{t+1}$ respectively.

\subsection{A bound on empowerment}
\label{sec:methods:efficient_estimation_of_empowerment}
The empowerment value of a state $\nowstate$ has been defined as the channel capacity between the action $\baction$ and the following state $\succstate$  \citep{klyubin2005empowerment},
\eq{
    \emp(\nowstate) = \max_{\source}\, \mi{\succstate, \baction}{\nowstate}. \numberthis \label{eq:empowerment}
}
Here, $\mathcal{I}$ is the mutual information. 
In this context $\source$ is a policy, a \emph{source distribution}.
It is distinct from the empowerment-maximising policy~$\policy$.
By definition, empowerment is the maximum information (measured in \emph{nats}) an agent can emit to its environment by changing the state through its actions.
We will refer to the maximising policy $\optimalsource = \arg\max_{\source}\, \mi{\succstate, \baction}{\nowstate}$ as the \emph{optimal source}.
Note that this problem can be interpreted as a stochastic optimal-control problem \citep{stengel2012optimal}, where we are trying to find a control policy that maximises an information-theoretic quantity of the environment.

To tackle empowerment, consider the mutual information in \cref{eq:empowerment}.
It is defined as 
\eq{
    \mi{\succstate, \nowaction}{\nowstate} 
        :=& \kl{\jointtrans}{\margtrans\,\source{\nowaction}{\nowstate}} \\
        =& \iint\!  \jointtrans \ln \frac{\jointtrans}{\margtrans \,\sourcetrans}\dint{\succstate} \dint{\nowaction},
}
where we use a source distribution $\source$ as policy. 
The intractability of \cref{eq:empowerment} is due to the \emph{marginal transition} 
\begin{align*}
	\margtrans = \int \sourcetrans \, \jointtrans \dint{\nowaction}.
\end{align*}
We avoid the integral over all actions by switching to the \emph{planning distribution} $\planning$:
\eq{
    \mi{\succstate, \nowaction}{\nowstate} \!
        &= \!\!\iint \! \jointtrans\! \ln \frac{\cancel{\margtrans}\, \planning}{\cancel{\margtrans}\,\sourcetrans}\dint{\succstate} \dint{\nowaction}.
}
While the planning distribution is equally intractable, it is easier to employ a variational approximation $\apxplanning$. This leads to the bound introduced by \cite{barber2003im}:
\eq{
    \mi{\succstate, \nowaction}{\nowstate} 
        &\ge  \iint  \jointtrans \ln \frac{\apxplanning}{\sourcetrans}\dint{\succstate} \dint{\nowaction} \numberthis \label{eq:vi_bound}\\
        &=: \mibound{\succstate, \nowaction}{\nowstate}.
}
The gap in \cref{eq:vi_bound} can be expressed as
\eq{
	\mi - \mibound 	=   \expc[\succstate \sim \margtrans]{\kl{\planning}{\apxplanning}},\numberthis\label{eq:gap}
}
cf.\ \cref{app:bound} for details. 
Hence, as $\mi$ is constant \wrt $q$, maximising the bound $\mibound$ \wrt $q$ and $\source$ simultaneously maximises the mutual information while keeping the variational approximation $\apxplanning$ close to the true planning distribution $\planning$.

If the variational approximation is learnt well and chosen to be sufficiently expressive to represent the true planning distribution, the bound will be tight.
Quite a few means to improve upon variational approximations have been proposed recently, e.g.\ by \cite{rezende2015flows,burda2015importance,kingma2016improving}.

Replacing $\mi$ with $\mibound$, we achieve a lower bound on empowerment:
\eq{
    \empbound(\nowstate) :=& \max_{\source}\mibound{\succstate, \nowaction}{\nowstate} \numberthis \label{eq:emp_bound} \le \emp(\nowstate).
}

\subsection{Efficient mutual information optimisation}
\label{sub:efficient_mi}
\Cref{eq:emp_bound} establishes a lower bound on empowerment which relies on the estimator $\mibound$ from \cref{eq:vi_bound} for mutual information.
This section provides a new, efficient method to exploit this bound.

The key assumption is that we can efficiently compute
\eq{
	\pd{}{\sourceplanningpars}\mibound{\succstate, \nowaction}{\nowstate} = 	\pd{}{\theta}\expc[\jointtrans]{ \ln \frac{\apxplanning}{\sourcetrans} },
}
where $\sourceplanningpars$ denotes the joint of parameters $\source$ and $q$.

If both the system dynamics and the source can be sampled efficiently, we can estimate the gradients of the mutual information bound via Monte-Carlo sampling and the reparametrisation trick \citep{kingma2014auto,RezendeMW14}, \ie 
\eq{
	\pd{}{\sourceplanningpars} \mibound{\succstate, \nowaction}{\nowstate}
	\approx \frac{1}{N} \sum_{n=1}^{N} \pd{}{\sourceplanningpars}\left[ \ln \q{\nowaction^{(n)}}{\nowstate, \succstate\,^{(n)}} \right.\\ 
    \left. -\ln \source{\nowaction^{(n)}}{\nowstate} \right],
}
where $\nowaction^{(n)} \sim \source{\nowaction}{\nowstate}$ and $\succstate\,^{(n)} \sim \p{\succstate}{\nowstate, \nowaction^{(n)}}$ as in \cref{eq:joint_dynamics}.
Here, we assume that $\pd{\succstate}{\nowaction}$, $\pd{\succstate}{\nowstate}$ and $\pd{\nowaction}{\sourceplanningpars}$ can be efficiently estimated.

\cite{mohamed2015variational} report a model-free optimisation of the same bound $\mibound$.
In this case optimising $\mibound$ for $\source$ collapses to maximising the entropy of $\source$, which requires them to constrain said entropy.
In contrast, our sampling process couples $q$ and $\source$:
the samples used to evaluate $q$ are drawn using $\source$ and system dynamics---in particular no rollouts---and the entropy of $\source$ is balanced by the negative entropy of $\q$. \cite{mohamed2015variational} create this coupling by minimising a squared error containing $\q$ and the approximation of $\source$.


Our methodology allows for principled joint optimisation of planning and source distribution via backpropagation \citep{rumelhart1986learning}, for which, to the best of our knowledge, no experimental results have been reported previously.


\subsection{Exploiting empowerment}
\label{sec:methods:empowerment_maximising_agents}
The findings of the previous section allow for efficient learning of the optimal source $\optimalsource$, which in turn allows us to estimate empowerment.
The main goal of this is not to obtain a certain policy, but to estimate the empowerment value of states.
As the empowerment value can be perceived as an unsupervised value of each state, it can be used to train agents which proceed towards empowering states.
We hence use negative empowerment as a cost function in a stochastic optimal-control framework \citep{stengel2012optimal}.
Let such an agent be represented by a policy $\policy$ with parameters $\policypars$.
We then train it to minimise the cost function
\eq{
     \Cost(\policy) := -\expc[\policy]{\sum_{t=1}^T \empbound(\bstate_t)}  
    \approx& \, -\frac{1}{M} \sum_{m=1}^M \sum_{t=1}^T \empbound\left(\bstatet^{(m)}\right) \numberthis \label{eq:empowering_cost}.
}
The right-hand side approximation of $\Cost(\policy)$ is computed by a two-stage sampling process:
the samples $\bstatet^{(m)}$ are sampled according to the system dynamics model and the policy $\pi$.
Within the evaluation of $\empbound\bigl(\bstatet^{(m)}\bigr)$ according to \cref{sub:efficient_mi}, we take $\bstatet^{(m)}$ as a seed for further sampling one step according to the source distribution $\source$.
For protecting the policy from getting stuck at suboptimal solutions we introduce a KL divergence between the policy $\policy$ and a standard normal distribution.
A parameter $\beta$ weights the cost against this regulariser.
The procedure is summarised in \cref{alg:training}.
The assumptions of \cref{sub:efficient_mi} allow us to efficiently estimate all gradients of $\cost{\policy}$ via, e.g.,
reparametrisation.

We want to stress two properties where our method differs.
Firstly, the availability of a differentiable model lets us propagate through the transitions, enabling the agent to trade short term cost for future reward.
Secondly, the time horizon $T$ is a hyper-parameter only of the training of $\policy$, and setting it to a different value does not require re-estimation of $\apxplanning$ and $\empbound$.

This allows us to amortise the exploitation of empowerment over an arbitrary horizon into a single, fixed-computation time policy $\policy$, granting real-time applicability.

\begin{algorithm*}[t!]
		\caption{Joint training of policy $\policy$, source $\source$ and approx.\ planning distribution $\apxplanning$}
	\begin{algorithmic}
		\Require dynamics $\p{\bstate_{t+1}}{\bstate_t, \baction_t}$, cumulation horizon $T$, initialisations for $\policy, \source,$ and $\q$
		\Repeat 
			\For{$m=1:M$}\Comment{Estimate cumulated empowerment $\Cost$, \cref{eq:empowering_cost}}
				\State {$\policy$-step: Sample dynamics with policy ${\policy}$:}
				\State \hspace{\algorithmicindent}{$ \bstate_{1:T}^{(m)}, \baction_{1:T-1}^{(m)} \sim \transition{\bstate_1} \prod_{t=1}^{T-1} \transition{\bstate_{t+1}}{\bactiont,\bstatet} \policy{\bactiont}{\bstatet}$ }
				\For{$t=1:T$}
					%\State {estimate $\empbound\left(\bstatet^{(m)}\right)$:}
					\State $\source$-step: Sample one step with policy ${\source}$: 
					\State \hspace{\algorithmicindent}{$\bactiont^{\source} \sim \source{\bactiont}{\bstatet^{(m)}}, \bstate_{t+1}^\omega \sim \transition{\bstate_{t+1}}{\bactiont^\omega,\bstatet^{(m)}}$} 
					\State {$\hat{\mathcal{I}}_t^m \leftarrow \ln {\plan{\bactiont^\omega}{\bstate_{t+1}^\omega, \bstatet^{(m)}}{\theta}} - \ln\source{\bactiont^\omega}{\bstatet^{(m)}}$
					\Comment{One-shot MI, \cref{eq:vi_bound,eq:emp_bound}}}
				\EndFor
			\EndFor
			\State {$\Cost \leftarrow \sum_m\sum_t \left[ \beta \hat{\mathcal{I}}_t^m + \kl{\policy{\bactiont^{(m)}}{\bstatet^{(m)}}}{\policy_0} \right]$\Comment{Cost and KL towards policy prior $\policy_0$}}
			\State {$\theta \leftarrow \theta + \lambda_\theta\nabla_{\!\theta}\, \mathcal{C}$ \Comment{gradient ascent in $\source$ and $q$ with some learning rate $\lambda$}}
			\State {$\chi \leftarrow \chi + \lambda_\chi\nabla_{\!\chi} \,\mathcal{C}$ \Comment{gradient ascent in \policy\ with some learning rate $\lambda$}	}	
		\Until{convergence}

	\end{algorithmic}

	\label{alg:training}
\end{algorithm*}



\subsection{Learning Markovian and differentiable models from data}
\label{sec:methods:learning_markovian_and_differentiable_models_from_data}
The methods presented so far build on a key assumption: the availability of a high-quality Markovian system dynamics model that (i) is differentiable, and (ii) can be evaluated efficiently.

In cases where any of these assumptions is not met, we learn the required model\footnote{We write, e.g., \bobsseq\ for \bobsTs\ to reduce notational clutter.}
\eq{
	\p{\bobsseq}{\bactionseq} = \int &\p{\bobs_1}{\bstate_1} \, \initial{\bstate_1}\\& \prod_{t=2}^T \p{\bobst}{\bstate_t} \, \p{\bstate_t}{\bstate_{t-1} , \baction_{t-1}} \dint \bstateseq
}

from a data set of \emph{observations} and controls through a slight modification of the recently proposed Deep Variational Bayes Filters (DVBF; \cite{karls2016deep}); for details we refer to \cref{app:dvbf}.
This model has been shown to discover physically plausible system dynamics from raw sensor readings through the maximisation of the \emph{evidence lower bound} (ELBO) on the log-likelihood,
\eq{
    &\ln \p{\bobsseq}{\bactionseq} \geq\elbo(\bobsseq, \bactionseq)\ \\= 
        \, &\expc[q]{\ln \p{\bobsseq}{\bstateseq}} +\kl{\q{\bstateseq}{\bobsseq, \bactionseq}}{\p{\bstateseq}{\bactionseq}}.
}

By design, the learnt transition distribution can be reparametrised, as is necessary in \cref{sub:efficient_mi}.

When evaluating the learnt empowerment-maximising policy $\policy$ from \cref{sec:methods:empowerment_maximising_agents} in the real environment we make use of the observations and the recognition network $\q{\bstateseq}{\bobsseq, \bactionseq}$ from above.
This network acts as a filter for the latent state and keeps it from diverging from the true state of the environment.
This recognition network has the same complexity as the policy thus does not influence its real-time applicability.

\subsection{$n$-step empowerment}

Empowerment can also be computed over a horizon of actions and transition steps, it is then called \emph{$n$-step empowerment}.
Instead of maximising the mutual information between the taken action $\bactiont$ and the next state $\bstate_{t+1}$ given the current state $\bstatet$, we maximise the mutual information between the \emph{sequence} of $n$ actions $\baction_{t:t+n-1}$ and the consequential state $\bstate_{t+n}$, given the starting state $\bstatet$.
We can apply the same methodology as in the last section:
we simply switch from a single-step variational planning distribution $\q{\bactiont}{\bstatet, \bstate_{t+1}}$ to an $n$-step planning distribution $\q{\baction_{t:t+n-1}}{\bstatet, \bstate_{t+n}}$.

When experimenting $n$-step empowerment in section \cref{sec:experiments}, we keep the source distribution parametrised by one fully connected network, whereas we factorise the planning distribution, similarly to \cite{mohamed2015variational}:
\eq{
    &\q{\baction_{t:t+n-1}}{\bstate_{t+n}, \bstatet}\\ =\, &\q{\bactiont}{\bstate_{t+n}, \bstatet} \prod_{k=0}^{n-1} \q{\baction_{t+k+1}}{\bstate_{t+n}, \baction_{t+k}, \bstatet}.
}


==> related.tex <==
\section{Related Work}
\label{sec:related-work}
Since empowerment has been introduced \citep{klyubin2005empowerment,salge2014empowerment}, several works have attempted to provide a concrete and scalable implementation.
The mutual information component is notoriously hard to calculate.
The early literature \citep{klyubin2005empowerment, klyubin2008options} circumvents these issues by operating in discrete-action state spaces and using the Blahut--Arimoto algorithm \citep{blahut1972computation}
which extensively samples action and state space and uses a iterative scheme to update the source distribution.
\cite{jung_empowerment_2011} take one step further by fitting the transitions with Gaussian processes and approximating empowerment by Monte-Carlo integration.
They introduce empowerment for continuous state spaces but still needs discrete actions and furthermore requires a large sample size to provide satisfactory solutions. 
\cite{salge_approximation_2013} solve the intractability by linearising the dynamic systems which enables the use of well-known closed-form solutions.
%
More recently, \cite{mohamed2015variational} proposed a scalable approach by maximising a lower bound on the mutual information.
Their work does not assume or learn a model of the environment and is restricted to an open-loop setting.
The term \emph{unsupervised control} was recently used by \cite{gregor2016variational}, who also resorted to an information-theoretic reward.
Unlike \cite{mohamed2015variational}, the authors targeted closed-loop policies with two algorithms.
The first, based on options \citep{sutton1999between}, is hard to train according to the authors and is restricted to linear function approximation. The second algorithm drops the option framework in order to overcome the aforementioned limitations. It is important to note that both algorithms are model-free, which constitutes the main difference with our approach.

Empowerment can be perceived as a member of a greater family of reward functions, reassembling intrinsic motivations \citep{singh2004intrinsically}.
We refer the reader to an excellent discussion on intrinsic motivation and a more thorough overview from \cite{oudeyer2008can};
here we present a few notable works.
Often the goal is to trigger explorative behaviour in the agent.
\cite{schmidhuber1991curious,schmidhuber2010formal} proposed to use a formalised notion of interestingness and curiosity.
%
\cite{bellemare2016unifying} show that increasing the value of under-visited states is related to information gain.
%
It has also been shown that a notion of \emph{surprise}, quantifying the degree to which an agent is observing something unexpected, can improve reinforcement learning \citep{itti2006bayesian,achiam2017surprise}.
One central notion in our work, the mutual information, has also been used to estimate information gain by \cite{houthooft2016vime} which is then integrated with the task-specific reward function.
Artificial creativity has been used to create games that aim to make an agent improve upon its current capabilities \citep{schmidhuber2013powerplay,sukhbaatar2017intrinsic}.

